A Tail-Index Analysis of Stochastic Gradient Noise in Deep Neural Networks

The gradient noise (GN) in the stochastic gradient descent (SGD) algorithm is often considered to be Gaussian in the large data regime by assuming that the classical central limit theorem (CLT) kicks in. This assumption is often made for mathematical convenience, since it enables SGD to be analyzed as a stochastic differential equation (SDE) driven by a Brownian motion. We argue that the Gaussianity assumption might fail to hold in deep learning settings and hence render the Brownian motion-based analyses inappropriate. Inspired by non-Gaussian natural phenomena, we consider the GN in a more general context and invoke the generalized CLT (GCLT), which suggests that the GN converges to a heavy-tailed $\alpha$-stable random variable. Accordingly, we propose to analyze SGD as an SDE driven by a L\'{e}vy motion. Such SDEs can incur `jumps', which force the SDE transition from narrow minima to wider minima, as proven by existing metastability theory. To validate the $\alpha$-stable assumption, we conduct extensive experiments on common deep learning architectures and show that in all settings, the GN is highly non-Gaussian and admits heavy-tails. We further investigate the tail behavior in varying network architectures and sizes, loss functions, and datasets. Our results open up a different perspective and shed more light on the belief that SGD prefers wide minima.

==> tech_bg.tex <==
%!TEX root = ./main.tex


\section{Stable distributions}
\label{sec:tech_bg}

{Central limit theorem (CLT) says that the sum of i.i.d. random variables with a finite second moment converges to a normal distribution if the number of summands grow. However, if the variables have heavy-tail, the second moment may not exist for instance if their density $p(x)$ has a power-law tail decreasing as $1/|x|^{\alpha+1}$ where $0 < \alpha < 2$ only $\alpha$-th moment exist with $\alpha<2$. In this case, generalized central limit theorem (GCLT) says that the sum of such variables will converge to a distribution called the  \emph{$\alpha$-stable} distribution instead as the number of summands grows (see e.g. \cite{fischer2010history}. In this work, we focus on the centered \emph{symmetric $\alpha$-stable} ($\sas$) distribution, which is a special case of $\alpha$-stable distributions that are symmetric around the origin.
}


We can view the $\sas$ distribution as a heavy-tailed generalization of a centered Gaussian distribution. The $\sas$ distributions are defined through their characteristic function via $X\sim \sas(\sigma) \iff \E[\exp(i \omega X)] = \exp(-|\sigma \omega|^\alpha)$. Even though, their probability density function do not admit a closed-form formula in general except in special cases, their density decays with a power law tail like $1/|x|^{\alpha+1}$ where $\alpha \in (0,2]$ is called the \emph{characteristic exponent} which determines the behavior of the distribution, as $\alpha$ gets smaller; the distribution has a heavier tail. In fact, the parameter $\alpha$ also determines the moments $\mathds{E}[|X|^p] < \infty$ if and only if $p<\alpha$; implying $X$ has infinite variance when $\alpha\neq 2$. The parameter $\sigma \in \mathds{R}_+$ is known as the \emph{scale} parameter and controls the spread of $X$ around $0$. We recover the Gaussian distribution ${\cal N}(0,2\sigma^2)$ as a special case of $\sas$ when $\alpha=2$.



